A Guide to Particle Advection Performance

The performance of particle advection-based flow visualization techniques is complex, since computational work can vary based on many factors, including number of particles, duration, and mesh type. Further, while many approaches have been introduced to optimize performance, the efficacy of a given approach can be similarly complex. In this work, we seek to establish a guide for particle advection performance by conducting a comprehensive survey of the area. We begin by identifying the building blocks for particle advection and establishing a simple cost model incorporating these building blocks. We then survey existing optimizations for particle advection, using two high-level categories: algorithmic optimizations and hardware efficiency. The sub-categories of algorithmic optimizations include solvers, cell locators, I/O efficiency, and precomputation, while the sub-categories of hardware efficiency all involve parallelism: shared-memory, distributed-memory, and hybrid. Finally, we conclude the survey by identifying current gaps in particle advection performance, and in particular on achieving a workflow for predicting performance under various optimizations.

==> portable.tex <==
\section{Performance Portability}
%
It is very common for users to run experiments on multiple computers.
%
Quiet commonly simulations are run on one cluster and analysis is run on other.
%
Also, when new generation of architectures replace existing ones,
applications need to be ported to execute with greater or at least the same efficiency 
on newer hardware.
%
It is not desirable for users to rewrite platform-specific,
optimized versions of code when such cases occur.
%
Hence, platform portability has become an important issue in saving costs incured
due to porting applications on newer hardware devices.
%
These problems are being addresed by programming libraries like
Kokkos~\cite{edwards2013kokkos}, RAJA~\cite{osti_1169830}, and
VTK-m~\cite{moreland2016vtk}.

The remainder of this section draws from a study I participated in on
the VTK-m software and its approach for portable performance.
%
The study has received a minor revision from the journal Parallel Computing,
and should be published later this year.
%
I performed all of the survey work described in this section,
including extracting all data for the tables and figures, and making
the tables and figures.
%
That said, much of the text was by my co-authors on the paper.

\subsection{VTK-m}

\input{vtkm-perf}


